A Game-Theoretic Approach for Hierarchical Epidemic Control

We design and analyze a multi-level game-theoretic model of hierarchical policy interventions for epidemic control, such as those in response to the COVID-19 pandemic. Our model captures the potentially mismatched priorities among a hierarchy of policy-makers (e.g., federal, state, and local governments) with respect to two cost components that have opposite dependence on the policy strength -- post-intervention infection rates and the socio-economic cost of policy implementation. Additionally, our model includes a crucial third factor in decisions: a cost of non-compliance with the policy-maker immediately above in the hierarchy, such as non-compliance of counties with state-level policies. We propose two novel algorithms for approximating solutions to such games. The first is based on best response dynamics (BRD), and exploits the tree structure of the game. The second combines quadratic integer programming (QIP), which enables us to collapse the two lowest levels of the game, with best response dynamics. Through extensive experiments, we show that our QIP-based approach significantly outperforms the BRD algorithm both in running time and the quality of equilibrium solutions. Finally, we apply the QIP-based algorithm to experiments based on both synthetic and real-world data under various parameter configurations and analyze the resulting (approximate) equilibria to gain insight into the impact of decentralization on overall welfare (measured as the negative sum of costs) as well as emergent properties like free-riding and fairness in cost distribution among policy-makers.

==> app_nynjdata.tex <==

\begin{figure}[ht!]
	\centering
%	\begin{subfigure}[t]{0.48\linewidth}
%	\includegraphics[width=0.99\linewidth]{figs/giniSymErrorBars.png}
%	\caption{Transport symmetry\label{fig:giniSym}}
%	\end{subfigure}
%    \begin{subfigure}[t]{0.48\linewidth}
	\includegraphics[scale=0.55]{figs/NYNJ_2_level/everage_county_alpha_gamma0.3.pdf}
%	\caption{Transport asymmetry (1 favorite County per State) \label{fig:giniaSym}}
%	\end{subfigure}
	\caption{The difference of the average counties' strategy profiles as a function of the government's strategy.\label{fig:NYNJ_gov}}
\end{figure}


We will now describe the real-world data sets that we used to construct the game environment for the experiments in Section~\ref{sec:ny-nj}.
We collected three sets of publicly available data on two states of the U.S.A., New York (NY) and New Jersey (NJ):
\begin{enumerate}[leftmargin=*,label=(\Alph*)]
    \item \label{roads} Two data sets on U.S. roads and road traffic published on September 30, 2020 by United States Department of Transportation, Federal Highway Administration (FHWA):
    \begin{enumerate}[leftmargin=*,label=(\arabic*)]
        \item \label{roadlength} \textbf{HM-20M 2019}\footnote{\url{https://www-fhwa-dot-gov.proxy.lib.umich.edu/policyinformation/statistics/2019/hm20m.cfm}}: This set tabulates Public Road Length (as of 2019) in kilometers for every U.S. state (rows), roads being categorized into RURAL and URBAN, and further sub-categorized into INTERSTATE, OTHER FREEWAYS AND EXPRESSWAYS, OTHER PRINCIPAL ARTERIAL, MINOR ARTERIAL, MAJOR COLLECTOR, MINOR COLLECTOR, and LOCAL (columns), these categories being called functional systems. We  only use data from the rows corresponding to the states of New York and New Jersey.
        \item \label{traffic} \textbf{VM-2 2019}\footnote{\url{https://www-fhwa-dot-gov.proxy.lib.umich.edu/policyinformation/statistics/2019/vm2.cfm}}: This set tabulates a quantification of Functional System Travel (as of 2019) in Annual Vehicle-Miles for each state and for each of the same categories and sub-categories of roads as 1. Again, we only use data from the rows corresponding to NY and NJ.
    \end{enumerate}
    \item \label{countypops} One data set on \textbf{County Population Totals} (2010-2019)\footnote{\url{https://www-census-gov.proxy.lib.umich.edu/data/datasets/time-series/demo/popest/2010s-counties-total.html}} released in March, 2020 by United States Census Bureau, Population division: For each state, a table records annual estimates of the resident population for counties in each state as of July 1 every year (rows) over the years 2010-2019 (columns), based on April 1 2010 U.S. census data. We only use data for all 62 counties of NY\footnote{Annual Estimates of the Resident Population for Counties in New York: April 1, 2010 to July 1, 2019 (CO-EST2019-ANNRES-36); Source: U.S. Census Bureau, Population Division; Release Date: March 2020} and all 21 counties NJ\footnote{Annual Estimates of the Resident Population for Counties in New Jersey: April 1, 2010 to July 1, 2019 (CO-EST2019-ANNRES-34); Source: U.S. Census Bureau, Population Division; Release Date: March 2020} for the year 2019 only.
\end{enumerate}

For our experiments, we imagine NY and NJ to form a closed system under a single federal government $g$, i.e. we consider an HECG where there are two States NY ($s_1$) and NJ ($s_2$) with 62 and 21 arbitrarily numbered Counties $\{c_1,c_2,\dots,c_{62}\}$ and $\{c_{63},c_{64},\dots,c_{83}\}$ under them respectively (see Figure~\ref{fig:model}).

For each County $c$, the share $\mu_c$ as defined in  Section~\ref{sec:game_model} is naturally given by the ratio of the population of County $c$ to the total population of all 83 Counties in the two States, all directly available from the data set~\ref{countypops}. Hence, we can obtain the shares of the States as  \[\mu_{s_1}=\sum_{i=1}^{62} \mu_{c_i}, \quad  \mu_{s_2}=\sum_{i=63}^{83} \mu_{c_i}.\] 
We also use all three data sets reported above to estimate the transport matrix $R = \{r_{cc'}\}_{c,c' \in \C}$ defined in Section~\ref{sec:infec}, as explained in the rest of this section. No other component of the model is estimated from these data sets.

First, we compute the \textit{traffic} on each road category in data sets~\ref{roads} as the ratio of vehicle-miles (from \textbf{VM-2 2019}) to road length (from \textbf{HM-20M 2019}). Then, we for each State $s \in \{s_1,s_2\}$, we compute 3 intermediate quantities that will give us the final transport matrix entries:
\begin{itemize}[leftmargin=*]
    \item $P_{\text{in-county}}(s)$, the ratio of the total traffic on the MAJOR COLLECTOR, MINOR COLLECTOR, and LOCAL road categories in State $s$ to the total traffic on all road categories in State $s$;
    \item $P_{\text{in-state}}(s)$, the ratio of the total traffic on the OTHER FREEWAYS AND EXPRESSWAYS, OTHER PRINCIPAL ARTERIAL, and MINOR ARTERIAL road categories in State $s$ to the total traffic on all road categories in State $s$;
    \item $P_{\text{between-states}}(s)$,  the ratio of the total traffic on the INTERSTATE road category in State $s$ to the total traffic on all road categories in State $s$.
\end{itemize}
Finally, we have
\begin{align*}
    r_{cc'} = \begin{cases}
    P_{\text{in-county}}(s) &\text{if $c = c'$},\\
    \frac{\mu_{c'}}{\mu_s} \cdot P_{\text{in-state}}(s) &\text{if $c\neq c'$, $c \in \chi(s)$, $c' \in \chi(s)$},\\
    \frac{\mu_{c'}}{1-\mu_s} \cdot P_{\text{between-states}}(s) &\text{if $c \in \chi(s)$, $c' \not\in \chi(s)$}.
    \end{cases}
\end{align*}



==> expts-omitted-fairness.tex <==
We will first take a closer look at the policies of the Counties and the resulting Gini coefficients for the experiments in Section~\ref{sec:exp-fairness}.

Under transport symmetry, Figures~\ref{fig:giniSymScatter} give us scatter plots of the realized Gini coefficient and the equilibrium policies of all Counties for each trial respectively; Figures~\ref{fig:gini_Asym_Scatter} and ~\ref{fig:gini_AsymAlphas} give us the corresponding scatter plots for the specific asymmetry where State 1 is the favorite destination.
\begin{figure}[h]
  \centering
  \includegraphics[scale=0.5]{figs/giniSymScatter.png}
    \caption{50 trials for each of 3 scenarios.}
  \label{fig:giniSymScatter}
\end{figure}
\begin{figure}[h]
  \centering
  \includegraphics[scale=0.5]{figs/ForGiniSymAlphas.png}
    \caption{50 trials for each of 3 scenarios.}
  \label{fig:giniSymAlphas}
\end{figure}
\begin{figure}[h]
  \centering
  \includegraphics[scale=0.4]{figs/Gini10counties_scatter_asym.pdf}
    \caption{30 trials for \textit{Aligned States}, 50 trials for each other scenario.}
  \label{fig:gini_Asym_Scatter}
\end{figure}
\begin{figure}[h]
  \centering
  \includegraphics[scale=0.4]{figs/Gini10counties_alphas_asym.pdf}
    \caption{30 trials for \textit{Aligned States}, 50 trials for each other scenario.}
  \label{fig:gini_AsymAlphas}
\end{figure}
Important observations on these scatter plots are that the values of the policies tend to be extreme and realized Gini coefficients seem to take on values from a small discrete set. The somewhat unique scenario is \textit{Aligned States} which has a higher variability or granularity in values for the symmetric setting --- a property that is lost under our specific asymmetry. 

==> expts-omitted.tex <==
\iffalse
We will first look at the variation in State 1 and 2's policies separately (Figures~\ref{fig:free-s1} and~\ref{fig:free-s2} respectively), rather than their difference, as we vary their shared non-compliance weight for the experimental set-up in Section~\ref{sec:exp-free-riding}. Recall that the initial infection rate of State 1 is fixed at $0.1$ and we wish to uncover conditions under which State 2 ends up free-riding, i.e. setting a weak policy ($\alpha_2$ close to $1$) while State 1 adopts a strong policy ($\alpha_1$ close to $0$).

The most striking observation is that State 1 maintains a maximally strict policy in equilibrium for a wide range of parameters (up to a compliance weight of around $0.15$ for all initial infection rates of State 2 studied here) while jumps to a fairly weak policy quickly over the same range.

\begin{figure}[ht!]
  \centering
  \includegraphics[scale=0.5]{figs/freeriding-s1.png}
    \caption{The Policy of State 1 (y-axis) as a function of non-compliance weight (x-axis) under transport symmetry. Each curve corresponds to a different initial infection rate for State 2 as specified in the legend.}
  \label{fig:free-s1}
\end{figure}

\begin{figure}[ht!]
  \centering
  \includegraphics[scale=0.5]{figs/freeriding-s2.png}
    \caption{The Policy of State 2 (y-axis) as a function of non-compliance weight (x-axis) under transport symmetry. Each curve corresponds to a different initial infection rate for State 2 as specified in the legend.}
  \label{fig:free-s2}
\end{figure}
\fi

Recall that we are in a setting with transport asymmetry where State 1 is the favorite destination, Figures~\ref{fig:free-asym-s1} and \ref{fig:free-asym-s2} provide insights into the behaviors of States 1 and 2 individually. Even when State 2's initial infection rate exceeds that of State 1 (which now has the moderate value $0.5$), State 1 now prefers to enforce no policy intervention for (almost) all values of its non-compliance weight while there is more variability in the equilibrium response of State 2.
\begin{figure}[ht!]
  \centering
  \includegraphics[scale=0.5]{figs/free-riding_asymState1.png}
    \caption{The Policy of State 1 (y-axis) as a function of non-compliance weight (x-axis) under our specific transport asymmetry. Each curve corresponds to a different initial infection rate for State 2 as specified in the legend.}
  \label{fig:free-asym-s1}
\end{figure}

\begin{figure}[ht!]
  \centering
  \includegraphics[scale=0.5]{figs/free-riding_asymState2.png}
    \caption{The Policy of State 2 (y-axis) as a function of non-compliance weight (x-axis) under our specific transport asymmetry. Each curve corresponds to a different initial infection rate for State 2 as specified in the legend.}
  \label{fig:free-asym-s2}
\end{figure}

Further, holding that non-compliance weight fixed at $0$, Figure~\ref{fig:State2_changeOverInitInf} depicts that on exceeding a threshold on its initial infection rate, State 2 chooses the weakest policy, now forcing State 1 to strengthen its own response and causing the reversal in Figure~\ref{fig:freeride_asym}.

\begin{figure}[ht!]
  \centering
  \includegraphics[scale=0.5]{figs/State2_change_w_initinf.png}
    \caption{The Policy of State 2 (y-axis) as a function of its own initial infection rate when its weight on the non-compliance cost is $0$ under our specific transport asymmetry.}
  \label{fig:State2_changeOverInitInf}
\end{figure}





==> figs/methods-appx.tex <==




\begin{figure}[ht!] 
	\centering
	\includegraphics[scale=0.35]{figs/syn_new.pdf}
	\caption{The number of best response steps (y-axis) as a function of the fraction of players that are best responding (x-axis). Each curve corresponds to a game with $n_2$ players (ranging from 5 to 45) in the second level which is also the lowest level of game. } 
	\label{fig:k}
\end{figure}


We conduct this experiment on a two-level game with one Government and a variable number $n_2$ of States. We focus on symmetric settings, i.e. all states have equal population, equal initial infections, and equal weight vectors. The transport matrix is also symmetric. Figure~\ref{fig:k} shows that setting $k_2 = n_2$ in Algorithm~\ref{alg:ne} (synchronous BRD) results in fastest convergence to equilibrium for several choices of $n_2$. %Besides, the algorithm \ref{alg:ne} converges very fast with in several rounds under this setting.
%In this simple example, if we pick $k = 1$, we can achieve the NE by just one step.
%For some games with a particular structure, such as a potential game, BRD with $k=1$ would be efficient to find the NE, and we do not need to evaluate the $\epsilon$ for each profile. 

% \sj{Feiran, can you add some description? Is this a two-level game where each person is as likely to go to each county and counties have the same size? what is the run-time in? Seconds? Number of Rounds? Can you change $\kappa_G$ to the correct symbol? What are the other weight values for the second level?}



% \sj{also please fix the figure similar to the other one in sec 3}

==> methods-appx.tex <==




\begin{figure}[ht!] 
	\centering
	\includegraphics[scale=0.38]{figs/syn_new.pdf}
	\caption{The number of best response steps (y-axis) as a function of the fraction of players that are best responding (x-axis). Each curve corresponds to a game with $n_2$ players (ranging from 5 to 45) in the second level which is also the lowest level of game. } 
	\label{fig:k}
\end{figure}

\mc{Omit asynchronous BRD altogether. Also from main paper.}
Recall that, in our general (potentially asynchronous) BRD approach, we pick uniformly at random 

We conducted a set of experiments on a two-level game (compliant setting) with one Government and a variable number of States $n_2=|\S|$ in order to . We focus on symmetric settings, i.e. all states have equal population, equal initial infections, and equal weight vectors. The transport matrix is also symmetric. Figure~\ref{fig:k} shows that setting $k_2 = |\S|$ in Algorithm~\ref{alg:ne} (synchronous BRD) results in fastest convergence to equilibrium for several choices of $|\S|$. %Besides, the algorithm \ref{alg:ne} converges very fast with in several rounds under this setting.
%In this simple example, if we pick $k = 1$, we can achieve the NE by just one step.
%For some games with a particular structure, such as a potential game, BRD with $k=1$ would be efficient to find the NE, and we do not need to evaluate the $\epsilon$ for each profile. 

% \sj{Feiran, can you add some description? Is this a two-level game where each person is as likely to go to each county and counties have the same size? what is the run-time in? Seconds? Number of Rounds? Can you change $\kappa_G$ to the correct symbol? What are the other weight values for the second level?}



% \sj{also please fix the figure similar to the other one in sec 3}
